Optimising the Performance of Convolutional Neural Networks across Computing Systems using Transfer Learning

The choice of convolutional routines (primitives) to implement neural networks has a tremendous impact on their inference performance (execution speed) on a given hardware platform. To optimise a neural network by primitive selection, the optimal primitive is identified for each layer of the network. This process requires a lengthy profiling stage, iterating over all the available primitives for each layer configuration, to measure their execution time on the target platform. Because each primitive exploits the hardware in different ways, new profiling is needed to obtain the best performance when moving to another platform. In this work, we propose to replace this prohibitively expensive profiling stage with a machine learning based approach of performance modeling. Our approach speeds up the optimisation time drastically. After training, our performance model can estimate the performance of convolutional primitives in any layer configuration. The time to optimise the execution of large neural networks via primitive selection is reduced from hours to just seconds. Our performance model is easily transferable to other target platforms. We demonstrate this by training a performance model on an Intel platform and performing transfer learning to AMD and ARM processor devices with minimal profiled samples.

==> doc/app_figs.tex <==
\begin{comment}
\begin{figure*}[t]
	\centering
	\bars{ds_size}{keys_lin_prim_red}{500,1000,1500,2000,2500,3000,3500,4000,4500}{\# Examples}
	\caption{The number of datapoints present in the primitive runtime dataset for each primitive. A mapping to the exact primitive names can be found in \cref{tab:ap_prims}.}\label{fig:exp_ds_size}
\end{figure*}
\end{comment}

\begin{comment}
\begin{figure*}[t]
	\centering
	\input{figures/nn_tikz_alt.tex}
	\caption{MdRAE -- the median relative absolute error (\cref{sec:ml_ml}) -- for the primitive runtime predictions of NN2 on the test set for the AMD and ARM machines.
		%	Error bars denote one standard deviation.
		A mapping to the specific primitive names can be found at \cref{tab:ap_prims}. Note that due to memory constraints on the ARM machine, not every primitive could be profiled, these primitives are left empty.
	}
	\label{fig:res_nns_alt}
\end{figure*}
\end{comment}

\begin{comment}
\begin{figure*}[t]
	\centering
	\input{figures/scatter_prims.tex}
	\caption{The predicted and actual runtimes of the test set for the Intel machine. The runtimes shown were taken as the mean predicted runtime across five repeated experiments. The dashed diagonal line denotes the points where the predictions equal the data.}
	\label{fig:res_predact}
\end{figure*}


\begin{figure*}[t]
	\centering
	\begin{subfigure}{1\textwidth}
		\corrbars{mean_nn_corr_test10}{std_nn_corr_test10}{keys_lin_prim_red}
		\caption{NN1}
	\end{subfigure}
	\begin{subfigure}{1\textwidth}
		\corrbars{mean_nn_full_corr_test10}{std_nn_full_corr_test10}{keys_lin_prim_red}
		\caption{NN2}
	\end{subfigure}
	\caption{
    	The correlation between the predicted and actual runtimes of the primitives of the test set for the Intel machine. Results are shown for the neural network models. 
    	%The error bars denote one standard deviation.
	}
	\label{fig:res_corr}
\end{figure*}
\end{comment}
